MixNorm: Test-Time Adaptation Through Online Normalization Estimation

We present a simple and effective way to estimate the batch-norm statistics during test time, to fast adapt a source model to target test samples. Known as Test-Time Adaptation, most prior works studying this task follow two assumptions in their evaluation where (1) test samples come together as a large batch, and (2) all from a single test distribution. However, in practice, these two assumptions may not stand, the reasons for which we propose two new evaluation settings where batch sizes are arbitrary and multiple distributions are considered. Unlike the previous methods that require a large batch of single distribution during test time to calculate stable batch-norm statistics, our method avoid any dependency on large online batches and is able to estimate accurate batch-norm statistics with a single sample. The proposed method significantly outperforms the State-Of-The-Art in the newly proposed settings in Test-Time Adaptation Task, and also demonstrates improvements in various other settings such as Source-Free Unsupervised Domain Adaptation and Zero-Shot Classification.

==> sections/experiments.tex <==
% For Testing-Time Adaptation Task, we follows the common protocol from \cite{wang2020tent} and evaluate our Mix-Norm Model with the standard benchmarks CIFAR10-C and ImageNet-C.
% \begin{itemize}
%     \item \textbf{CIFAR10-C (\cite{hendrycks2019benchmarking})}: \xuefeng{TODO: dataset introduction}
%     \item \textbf{ImageNet-C (\cite{hendrycks2019benchmarking})}: \xuefeng{TODO: dataset introduction}
% \end{itemize}
\textit{Datasets.} 
To evaluate our method's robustness to corruption, following TENT (\cite{wang2020tent}), we evaluated our method over the standard benchmarks CIFAR10-C and ImageNet-C (\cite{hendrycks2019benchmarking}). CIFAR10-C includes 75 subsets, composed of 15 types of corruptions at 5 severity levels. It comprises the 10,000 images, each of size 32x32 pixels, from the 10 classes in the CIFAR10 test set, but with each modified by the corresponding corruption type at certain severity level. Similarly, ImageNet-C is composed of a set of 75 common visual corruptions, applied to the original ImageNet validation set, with 50,000 images of 224x224 pixels from 1000 classes. 

For domain adaptation, we follow the experiment setup from \cite{wang2020tent} to use SVHN as the source domain and MNIST/MNIST-M/USPS as the target domains. Both SVHN, MNIST, MNIST-M and USPS are digits datasets with 10 classes, each with training/testing data size 73257/26032, 60000/10000, 60000/10000 and 7291/2007. 

For Zero-Shot Image Classification, we evaluate our method on CIFAR-10/100, ImageNet, STL-10, Birdsnap, FGVC Aircraft, Country211, Food101, SUN397 and Oxford-Pets. Details of these datasets are provided in the supplementary.

\textit{Baselines.} TODO

\textit{Implementation Details.} TODO

\subsection{Robustness to Corruptions}
    In order to understand the merit of our new method in real world scenarios, we introduce two new corruption conditions to the recent baseline work TENT. In TENT, error rates for each of the 15 corruption types at severity 5 are reported with fixed batch size of 200 on CIFAR10-C and 64 on ImageNet-C. In this paper, in addition to this standard protocol, we compare our method with TENT with two new conditions:
    \begin{itemize}
        \item Different Batch Size. In additional to the fixed 200/64 batch size in the standard protocol, we also compare our method with TENT at batch sizes at 1, 5, 8, 16, 32, 64, 100, 200.
        \item Mixed Distribution. In additional to the standard protocol where model's final error rate is averaged from 15 separate evaluation where in each evaluation only one type of corruption exists, we evaluate the models with all corruptions types shuffled and mixed together.  
    \end{itemize}

    \begin{figure}[ht]
    \begin{subfigure}{.5\textwidth}
      \centering
      % include first image
      \includegraphics[width=.8\linewidth]{figures/ImageNet-C Error Rates (Single Type, Severity=5).pdf}  
    %   \caption{Put your sub-caption here}
      \label{fig:sub-first}
    \end{subfigure}
    \begin{subfigure}{.5\textwidth}
      \centering
      % include second image
      \includegraphics[width=.8\linewidth]{figures/ImageNet-C Error Rates (Mixed Type, Severity=5).pdf}  
    %   \caption{Put your sub-caption here}
      \label{fig:sub-second}
    \end{subfigure}
    \begin{subfigure}{.5\textwidth}
      \centering
      % include first image
      \includegraphics[width=.8\linewidth]{figures/CIFAR-10C Error Rates (Single Type, Severity=5).pdf}  
    %   \caption{Put your sub-caption here}
      \label{fig:sub-first}
    \end{subfigure}
    \begin{subfigure}{.5\textwidth}
      \centering
      % include second image
      \includegraphics[width=.8\linewidth]{figures/CIFAR-10C Error Rates (Mixed Type, Severity=5).pdf}  
    %   \caption{Put your sub-caption here}
      \label{fig:sub-second}
    \end{subfigure}
    \caption{Comparison of our MixNorm and Mix-BatchNorm methods to the baseline method TENT in two different test time settings i) test samples come only from single type corruption; ii) test samples come from mixed types of corruptions. We report error rates using CIFAR-10C and ImageNet-C datasets.}
    \label{fig:robustness}
    \end{figure}

        Figure \ref{fig:robustness} shows our main results. blue curves represent the SOTA model TENT, the red and orange curves represent Mix-Norm model with and without fixed Batch-Norm weights, and the green curves represent the performance of MixNorm+TENT as described in Algorithm 2. As we previously discussed, Tent's performance drops as the batch size decreases, while Mixed-Norm's performance stays stable at any batch size.  
    
        Additional to the improvement to small batch size, Figure \ref{fig:robustness} also demonstrates the advantages of the Mix-Norm model when testing examples come from different distributions. 
        In \cite{wang2020tent}'s testing protocol, all testing examples are from the same corruption distribution, and therefore it can obtain reliable normalization statistics when batch size is large. However, when tested against samples from different distribution mixing together, such assumption can not hold and therefore Tent's performance can not outperform the Mix-Norm model, even tested with large batch size (up to 64 on ImageNet-C and up to 200 on CIFAR10-C).

\subsection{Ablation Studies}
In this section, we present the results of several ablations on architecture selection, ways of collecting normalization statistics and number of augmentations.
    \subsubsection{Architectures}
            \begin{figure}[ht]
            \begin{subfigure}{.5\textwidth}
              \centering
              % include first image
              \includegraphics[width=.8\linewidth]{figures/CIFAR-10C Error Rates (Single Type, Severity=5) (1).pdf}  
            %   \caption{Put your sub-caption here}
            %   \label{fig:sub-first}
            \end{subfigure}
            \begin{subfigure}{.5\textwidth}
              \centering
              % include second image
              \includegraphics[width=.8\linewidth]{figures/CIFAR-10C Error Rates (Mixed Type, Severity=5) (1).pdf}  
              %\caption{Put your sub-caption here}
              %\label{fig:sub-second}
            \end{subfigure}
            \caption{Comparison of our MixNorm and Mix-BatchNorm methods to the baseline method TENT, with different backbone architecture (WideResNet40)}
            \label{fig:arch}
            \end{figure}
            In Figure \ref{fig:arch} we demonstrate the CIFAR10-C results where both TENT and Mix-Norm adopt a more powerful backbone WideResNet40 compare to the WideResNet28 used in Figure \ref{fig:robustness}. The results shows Mix-Norm maintains its advantages on different architectures and at different accuracy ranges.
    
    \subsubsection{Normalization Statistics Estimation}
        In Table \ref{fig:ablation} we present the ablation study on different ways to collect normalization parameters. As shown in the table, using either global statistics ('Moving Global Norm') or local statistics ('Augmentation Norm') do not have good performance. However, combining the global and local statistics gives better performance than both.
    \subsubsection{Augmentations}
        In Table \ref{fig:augmentation}, it shows one augmentation is enough the get good performance, and the number of augmentation in local statistics calculation does not have significant influence on performance. Therefore, we just use one augmentation for faster computation. 


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{cccccllll}
\cline{1-5}
\multirow{2}{*}{Experiment Name} & \multicolumn{3}{c}{Way of Collecting Means \& Vars}                & \multirow{2}{*}{Error Rate} &\\ \cline{2-4}
                                 & Moving Speed         & Global Scale         & Local Scale          &                             &\\ \cline{1-5}
Instance Norm                    & 0                    & 0                    & 1                    & 78.21\%                     &\\
Augmentation (Local) Norm        & 0                    & 0                    & 1                    & 68.73\%                     &\\ \cline{1-5}
Fixed Global Norm                & 0                    & 1                    & 0                    & 50.50\%                     &\\
Moving Global Norm               & 0.001                & 1                    & 0                    & 38.45\%                     &\\ \cline{1-5}
Mixed Norm                       & 0.001                & 0.95                 & 0.95                 & 34.45\%                     &\\
Mixed Norm                       & 0.001                & 0.9                  & 0.1                  & 32.66\%                     &\\
Mixed Norm                       & 0.001                & 0.8                  & 0.2                  & \textbf{31.96\%}            &\\ \cline{1-5}
Mixed Norm  w/ fixed params                    & 0.001                & 0.8                  & 0.2                  & \textbf{32.01\%}            &\\
\multicolumn{1}{l}{}             & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}        &
\end{tabular}
 \caption{Ablation studies on different ways to collect normalization statistics, tested with CIFAR10-C, mixed corruption examples.}
    \label{fig:ablation}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{cccllllll}
\cline{1-3}
\multirow{2}{*}{Experiment Name} & \multirow{2}{*}{Number of Augmentation} & \multirow{2}{*}{Error Rate} &\\
                                 &                                         &                             &\\ \cline{1-3}
\textbf{Mixed Norm}              & \textbf{1}                              & \textbf{58.16\%}            &\\
Mixed Norm                       & 3                                       & 58.33\%                     &\\
Mixed Norm                       & 5                                       & 58.35\%                     &\\
Mixed Norm                       & 7                                       & 58.44\%                     &\\
Mixed Norm                       & 9                                       & 58.49\%                     &\\
Mixed Norm                       & 15                                      & 58.56\%                     &\\
\end{tabular}
\caption{Ablation studies on the effect of number of augmentations to collect normalization statistics, tested with ImageNet-C, mixed corruption examples.}
    \label{fig:augmentation}
\end{table}

\begin{table}[!ht]
    \centering
    \begin{tabular}{cclll}
    \hline
    Model      & CIFAR-100 & \multicolumn{1}{c}{CIFAR-10} & \multicolumn{1}{c}{STL-10} & \multicolumn{1}{c}{ImageNet} \\ \hline
    CLIP (ViT) & 64.21\%   & -                         & -                        & -                            \\
    Mixed-Norm & 64.67\%   & -                         & -                        & -                           \\
    \\ \hline
    Model      & Birdsnap & \multicolumn{1}{c}{Country211} & \multicolumn{1}{c}{Food101} & \multicolumn{1}{c}{Sun397} \\ \hline
    CLIP (ViT) & 64.21\%   & -                         & -                        & -                            \\
    Mixed-Norm & 64.67\%   & -                         & -                        & -                           
    \end{tabular}
    \caption{Zero-Shot Experiment. We replaced the Layer-Norm layers in the pre-trained CLIP Visual-Transformer weights and tested it under the zero-shot setting on the standard benchmarks. Result shows Mix-Norm improved the CLIP performance}
    \label{clip-vit}
    \end{table}

\subsection{Testing-Time Adaptation in Zero-Shot Learning Setting}
    In Table \ref{clip-vit} and \ref{clip-rn}, we replace the Layer-Norm layers from the pre-trained CLIP models, with backbone architectures of both Visual-Transformer and ResNet-50. The result shows Mix-Norm improved the CLIP's zero-shot learning performance in both case on CIFAR-100. 
    
    
    
    \begin{table}[!ht]
    \centering
    \begin{tabular}{cclll}\hline
    Model       & CIFAR-100 & \multicolumn{1}{c}{CIFAR-10} & \multicolumn{1}{c}{STL-10} & \multicolumn{1}{c}{ImageNet} \\ \hline
    CLIP (RN50) & 40.97\%   & -                         & -                        & -                            \\
    Mixed-Norm  & 43.51\%   & -                         & -                        & -                           
    \\
    \\ \hline
    Model      & Birdsnap & \multicolumn{1}{c}{Country211} & \multicolumn{1}{c}{Food101} & \multicolumn{1}{c}{Sun397} \\ \hline
    CLIP (RN50) & 40.97\%   & -                         & -                        & -                            \\
    Mixed-Norm  & 43.51\%   & -                         & -                        & -                           
    \end{tabular}
    \caption{Zero-Shot Experiment. We replaced the Layer-Norm layers in the pre-trained CLIP ResNet-50 weights and tested it under the zero-shot setting on the standard benchmarks. Result shows Mix-Norm improved the CLIP performance}
    \label{clip-rn}
    \end{table}

\subsection{Source-Free Unsupervised Domain Adaptation}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\begin{tabular}{ccccccc}
\multirow{2}{*}{Method} & \multirow{2}{*}{Source} & \multirow{2}{*}{Target} & Epoches         & \multicolumn{3}{c}{Error}                                                      \\ \cline{4-7} 
                        &                         &                         & Source + Target & MNIST                    & MNIST-M                  & USPS                     \\ \hline
Source                  & train                   & \multicolumn{1}{l}{}    & -               & \multicolumn{1}{r}{18.2} & \multicolumn{1}{r}{39.7} & \multicolumn{1}{r}{19.3} \\
RG                      & train                   & train                   & 10+10           & \multicolumn{1}{r}{15}   & \multicolumn{1}{r}{33.4} & \multicolumn{1}{r}{18.9} \\
UDA-SS                  & train                   & train                   & 10+10           & 11.1                     & 22.2                     & 18.4                     \\
BN                      & \multicolumn{1}{l}{}    & test                    & 0+1             & 15.7                     & 39.7                     & 18                       \\
TENT                    & \multicolumn{1}{l}{}    & test                    & 0+1             & 10                       & 37                       & 16.3                     \\
Mix-BN                  & \multicolumn{1}{l}{}    & test                    & 0+10            & -                        & -                        & -                       
\end{tabular}
\caption{Digit domain adaptation from SVHN to MNIST/MNIST-M/USPS. Source-free adaptation is
not only feasible, but more efficient.}
\end{table}

==> sections/introduction.tex <==
Deep learning models have brought tremendous performance improvements over many different domains (\cite{krizhevsky2012imagenet,he2016deep,deng2009imagenet}) in recent years. 
However, we often find that a well-trained model performs unexpectedly poorly in real-world settings. Many factors are in play here but one of the most probable causes stems from a domain shift from the training data~\cite{quinonero2009dataset}. 

encounters the performance drop in real production environment. One possible reason could be the domain shift between training data and the practical testing data, as described by \cite{quinonero2009dataset}.
To study and simulate the domain shift in production environment and to evaluate the generalization ability of deep learning models, many benchmarks have been proposed (\cite{saenko2010adapting,peng2017visda,hendrycks2019benchmarking}). 
Figure \ref{fig:imagenet} demonstrates the samples from one of the benchmarks, ImageNet-C (\cite{hendrycks2019benchmarking}), that synthesis corruptions to ImageNet (\cite{deng2009imagenet}) testing images to simulate the test-time domain shift. 

To increase deep learning models' robustness towards domain shift, various methods have been developed in different settings, such as Domain Adaptation (\cite{patel2015visual}), Unsupervised Domain Adaptation(\cite{wilson2020survey}) and Source-Free Domain Adaptation(\cite{liang2020we}). Among all those different settings, the task of Fully Test-Time Adaptation (\cite{wang2020tent}) is one of the most challenging setting that has least requirement to deployment condition. With and only with access to a model that is pre-trained offline, the goal of Test-Time Adaptation (TTA) is to fast adapt the model into the testing domain while making predictions. The task is essentially Domain Adaptation plus three more challenging conditions:
\begin{itemize}
    \item \textbf{Online}: The model gets updated during making predictions, and access to each testing example only once.
    \item \textbf{Source-Free}: The model does not have access to training data after the offline training is done. It will only have access to the pre-trained weights. 
    \item \textbf{Unsupervised}: There is no label for testing examples. 
\end{itemize}

\begin{wrapfigure}{l}{0.5\textwidth}
  \begin{center}
    \includegraphics[width=0.5\textwidth]{figures/imagenet-c.png}
  \end{center}
  \caption{Examples from ImageNet-C dataset \cite{hendrycks2019benchmarking}. ImageNet-C contains 75 corrupted copies of the original ImageNet-1K test set, with 5 severity levels and 15 different corruption types. This dataset is used to simulate the distribution shift between training domain (original) and test domains (corrupted).}
  \label{fig:imagenet}
\end{wrapfigure}

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/imagenet-c.png}
%     \caption{Examples from ImageNet-C dataset \cite{hendrycks2019benchmarking}. ImageNet-C contains 75 corrupted copies of the original ImageNet-1K test set, with 5 severity levels and 15 different corruption types. This dataset is used to simulate the distribution shift between training domain (original) and test domains (corrupted).}
%     \label{fig:imagenet}
% \end{figure}

Several works have studied the Fully Test-Time Adaptation problem in the recent years (\cite{li2016revisiting,sun2020test,wang2020tent}). Existing methods focus on adapting the Batch Normalization Layers (\cite{ioffe2015batch}) in the deep learning models, and have significantly improved deep learning model's performance against test-time domain shift. Such Batch-Norm Layer based methods make two underlying assumptions to estimate stable normalization statistics during evaluation: 1) test data comes together in large batches; 2) all test data are from the same shifted distribution (single corruption types, single domain, etc). However, such assumptions might not be practical in production environment. Test examples might come from an arbitrary distribution, such as the domain shift caused by sample size, ways of collection, different types of corruptions. Also, test examples might come at any size, and the AI system might not have the freedom to postpone the prediction until it collect enough data to proceed the test-time adaptation algorithms. 

To decouple the dependency over large batch size and sole distribution, we propose to replace the Batch-Norm Layers with a novel MixNorm operation that perform adaptive prediction of the normalization statistics from single example. The novel MixNorm Layers looks at not only global statistics calculated from all history examples, but also local statistics calculated from incoming test sample and its spatial augmentations. The novel MixNorm method demonstrate significant improvement over the State-of-the-art methods TENT (\cite{wang2020tent}), especially in the two newly proposed evaluation protocols, where the all Test-Time Adaptation methods are evaluated at various batch sizes, and against mixture of test samples from different shifted domains. Besides the task of Test-Time Adaptation, the new MixNorm Layer also demonstrates improvement over various of task settings, such as source-free Domain Adaptation task and Zero-Shot Image Classification. 

Our contribution can be summarized in three folds:
\begin{itemize}
    \item We proposed two new evaluation protocols in the task of Test-Time Adaptation that decouple the less practical assumptions made by previous protocols. 
    \item We proposed a novel way to adaptive estimate the test-time normalization statistics from single example.
    \item We performed extensive experiments that demonstrate the effectiveness of the new MixNorm Layer in various tasks, such as Test-Time Adaptation, Source-Free Domain Adaptation and Zero-Shot Image Classification. 
\end{itemize}

==> sections/method.tex <==
\begin{algorithm}[H]
\SetAlgoLined
\KwInput{
Input Feature: $F\in R^{D\times H\times W}$
\\Augmentation Features of the same sample: $F'\in R^{N\times D\times H\times W}$
\\Training Set Mean $\mu^0$ and Variance $\sigma^0$
\\Exponential Moving Speed $\tau=0.001$
\\Mixing Scale $m=0.05$
\\Weights, Bias: $\alpha,\beta$
}
\textbf{Procedure:}\\
// Update $\mu$ and $\sigma$ with most recent sample \\
$\mu^{t+1} \gets (1-\tau)\mu^t + \tau F.mean(dim=(1,2))$ \\
$\sigma^{t+1} \gets (1-\tau)\sigma^t + \tau (F-\mu).var(dim=(1,2))$\\
// Calculate instance-agnostic statistics\\
$\mu_{global} \gets \mu^t $\\
$\sigma_{global} \gets \sigma^t $\\
// Calculate instance-dependent statistics\\
$\mu_{local} \gets F'.mean(dim=(0,2,3))$\\
$\sigma_{local} \gets (F'-\mu_{local}).var(dim=(0,2,3)$\\
// Mix Global and Local\\
$\mu_{mixed} \gets (1-m)\mu_{global} + m\mu_{local}$\\
$\sigma_{mixed} \gets (1-m)\sigma_{global} + m\sigma_{local}$ \\
// Calculate shifted f\\
$F \gets \alpha \frac{F-\mu_{mixed}}{\sigma_{mixed}}+\beta$\\
return $F$\\
\caption{Mix-Norm Update}
\label{algorithm}
\end{algorithm}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/all.pdf}
    \caption{Overall Single Example Testing-Time Adaptation Pipeline}
    \label{fig:all}
\end{figure}



\begin{algorithm}[H]
\SetAlgoLined
\KwInput{
Batch of Features: $F\in R^{B\times D\times H\times W}$
\\Augmentated Features of the same batch: $F'\in R^{B\times N\times D\times H\times W}$
\\Training Set Mean $\mu^0$ and Variance $\sigma^0$
\\Max Exponential Moving Speed $\tau_{max} = 0.9$
\\Mixing Scale $m=0.05$
\\Weights, Bias: $\alpha,\beta$
}
\textbf{Procedure:}\\
// Calculate Moving Speed based on Batch Size $B$\\
$\tau \gets \tau_{max}10^{-\frac{3}{B}}$\\
// Update $\mu$ and $\sigma$ with most recent sample \\
$\mu^{t+1} \gets (1-\tau)\mu^t + \tau F.mean(dim=(0,1,2))$ \\
$\sigma^{t+1} \gets (1-\tau)\sigma^t + \tau (F-\mu).var(dim=(0,1,2))$\\
// Update global statistics with current batch\\
$\mu_{global} \gets \mu^t $\\
$\sigma_{global} \gets \sigma^t $\\
// Calculate local statistics from augmentations\\
$\mu_{local} \gets F'.mean(dim=(0,1,3,4))$\\
$\sigma_{local} \gets (F'-\mu_{local}).var(dim=(0,1,3,4)$\\
// Mix Global and Local\\
$\mu_{mixed} \gets (1-m)\mu_{global} + m\mu_{local}$\\
$\sigma_{mixed} \gets (1-m)\sigma_{global} + m\sigma_{local}$ \\
// Calculate shifted f\\
$F \gets \alpha \frac{F-\mu_{mixed}}{\sigma_{mixed}}+\beta$\\
return $F$\\
\caption{Mix-Norm w/ Batch-Norm}
\label{algorithm}
\end{algorithm}

BN, TTT and TENT (\cite{li2016revisiting,sun2020test,wang2020tent}) proves that updating the batch-norm layers is an efficient and effective way to adapt the deep learning models towards the corrupted testing distribution. However, as we discussed above, it is usually necessary to have a relatively large batch of samples that come from the same distribution to make stable batch-norm statistic prediction. 

To achieve realistic TTA in true online setting, where testing example could come at any batch size, we propose a novel Mix-Norm layer that can predict accurate normalization statistics from just single example, and therefore decoupled the dependency over large batch size. 

Without a large batch to calculate empirical normalization statistics, our method predict the statistics from two source:
\begin{itemize}
    \item Global Statistics: The Batch-Norm layers from the pre-trained model store the statistics from training distribution. In our Mix-Norm layer, we use this training domain statistics as an global anchor point. The global statistics will be initialized by the training domain statistics, and will be updated by the exponential moving average of the online testing sample. 
    \item Local Statistics: We use create an additional augmented view of the single example to form a small 2-example batch. We calculate the empirical statistics from this simulated batch to capture the local distribution shift for the particular example. The augmentation types are spatial augmentations include random-resized-crop and random-flipping. 
\end{itemize}

In a typical deep learning model such as ResNet (\cite{he2016deep}) or WideResNet (\cite{zagoruyko2016wide}), there will be multiple batch-norm layers across the whole backbone network. In Figure \ref{fig:all} and Figure \ref{fig:mixnorm}, we focus on the operation in one of such layers to demonstrate our method. 

As shown in Figure \ref{fig:all}, each example $X$ comes along with its augmented view $X'$. After the encode of the network layers previous to our Mix-Norm layer, input images $X, X'\in \mathbb{R}^{3\times224\times224}$ become feature tensor $F,F'\in\mathbb{R}^{D\times H\times W}$. For simplicity, we denote the $i$-th row, $j$-th column of $F, F'$ to be $F_{i,j},F'_{i,j}\in\mathbb{R}^{D}$.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/mixnorm.pdf}
    \caption{Mix-Norm Layer}
    \label{fig:mixnorm}
\end{figure}

As demonstrated in Figure \ref{fig:mixnorm}, our global statistics $\mu^t, \sigma^t$ are initialized with training set statistics, copied from the batch-norm layers in the pre-trained network:
\begin{align*}
    \mu^0 &= \mu^{training}\\
    \sigma^0 &= \sigma^{training},
\end{align*}
and they will be slowly updated by the statistics on each new example:
\begin{align*}
    \mu^{t+1} &= (1-\tau)\mu^{t}+\tau \mu \\
    \sigma^{t+1} &= (1-\tau)\sigma^{t}+\tau \sigma,
\end{align*}
where $\tau$ is the exponential moving speed, and $\mu$ and $\sigma$ are the means and variances from $F$:
\begin{align*}
    \mu &= \frac{\sum_{i=0}^H\sum_{j=0}^W F_{ij}}{HW} \\
    \sigma &= \frac{\sum_{i=0}^H\sum_{j=0}^W (F_{ij}-\mu)^2}{HW}.
\end{align*}
On the other hand, we calculate the local statistics $\mu_{local},\sigma_{local}$ by looking at both $F,F'$:
\begin{align*}
    \mu_{local} &= \frac{\sum_{F^*\in\{F,F'\}}\sum_{i=0}^H\sum_{j=0}^W F^*_{ij}}{2HW} \\
    \sigma_{local} &= \frac{\sum_{F^*\in\{F,F'\}}\sum_{i=0}^H\sum_{j=0}^W (F^*_{ij}-\mu_{local})^2}{2HW}
\end{align*}
Rename $\mu^{t+1},\sigma^{t+1}$ to be $\mu_{global},\sigma_{global}$, we obtained our final statistics:
\begin{align*}
    \mu_{mixed} &= (1-m)\mu_{global} + m\mu_{local}\\
    \sigma_{mixed} &= (1-m)\sigma_{global} + m\sigma_{local}.
\end{align*}
Finally, with $\mu_{mixed}, \sigma_{mixed}$, we can perform the normalization operation, and forward the resulted $F,F'$ to next layers:
\begin{align*}
    F &= \alpha\frac{F-\mu_{mixed}}{\epsilon+\sqrt{\sigma_{mixed}}}+\beta\\
    F' &= \alpha\frac{F'-\mu_{mixed}}{\epsilon+\sqrt{\sigma_{mixed}}}+\beta,
\end{align*}
where $\alpha,\beta,\epsilon$ are the parameters copied from the pre-trained network batch-norm layers.
%The same process is also described in Algorithm \ref{algorithm}.


==> sections/related.tex <==
In practice, it is not very common for deep neural networks to adapt themselves to new incoming data. Once a model is trained on a training data (source), the model is deployed for inference and expected to perform similar to its performance on validation data (source). However, in practice, it is often the case where performance starts dropping over time. Recently, there has been new efforts to address this issue by adapting the models during inference (test) time.  
\subsection{Test-Time Adaptation} 
BN (\cite{li2016revisiting}) was one of the first works that explores the Test-Time-Adaptation task. It focuses on adapting the Batch-Norm Layers in the deep learning models. In a classic Batch-Norm module, the module collects running means and variances at training time from the training data, and uses the collected means and variance at test time. BN argues that when there are distribution shifts between training data and testing data, we should not keep using the training domain statistics. Instead, we should collect statistic directly from the online batch. BN demonstrates this simple trick of using online statistics is effective to handle the distribution shifts caused by corruptions. However, one clear drawback of the method is it requires relative large batches to obtain stable online statistics. 

Following the setting of BN (\cite{li2016revisiting}), TTT (\cite{sun2020test}) proposes to update not only the batch-norm statistics, but also the affine weights and biases. TTT performs a single step gradient update over the batch-norm parameters after each prediction, with an unsupervised loss defined by rotation prediction task. 

Following the setting of TTT\cite{sun2020test}, TENT (\cite{wang2020tent}) proposes to use entropy loss instead of rotation prediction loss and achieves the state-of-the-art performance on CIFAR10-C, CIFAR100-C and ImageNet-C dataset.

As we discussed above, most of the existing works in TTA follow the same evaluation protocol proposed by \cite{li2016revisiting}, where the models are tested with large batch of testing examples sampled from single type corruption. However, such an assumption is not realistic in practice, because the testing examples in real production environments could come at any batch size (in particular real time high performance inference platforms process 1 input at a time, see \cite{Anderson2021FirstGenerationIA}), or from any shifted distribution. 

\subsection{Source-Free Unsupervised Domain Adaptation}
\subsection{Zero-Shot Classification}

